Self-Supervised Visual Place Recognition Learning in Mobile Robots

Place recognition is a critical component in robot navigation that enables it to re-establish previously visited locations, and simultaneously use this information to correct the drift incurred in its dead-reckoned estimate. In this work, we develop a self-supervised approach to place recognition in robots. The task of visual loop-closure identification is cast as a metric learning problem, where the labels for positive and negative examples of loop-closures can be bootstrapped using a GPS-aided navigation solution that the robot already uses. By leveraging the synchronization between sensors, we show that we are able to learn an appropriate distance metric for arbitrary real-valued image descriptors (including state-of-the-art CNN models), that is specifically geared for visual place recognition in mobile robots. Furthermore, we show that the newly learned embedding can be particularly powerful in disambiguating visual scenes for the task of vision-based loop-closure identification in mobile robots.

==> tex/fig-loop-closure-comparison.tex <==
\begin{figure}[!h]
  \centering 
  {\renewcommand{\arraystretch}{0.4} %
    {\setlength{\tabcolsep}{1mm}
      \begin{tabular}{cc}
        \hspace{1mm}\myfiguretitle{Loop-closure candidates (\textit{Ours-fc7})}{6}
        &\hspace{1mm}\myfiguretitle{Loop-closure candidates (\textit{Places365-fc7})}{6}\\

        \includegraphics[width=0.48\columnwidth]{\SECPROJECTDIR/results/ours_closures.pdf}&
        \includegraphics[width=0.48\columnwidth]{\SECPROJECTDIR/results/seqslam_closures.pdf}
      \end{tabular}}}
  \mycaption{Qualitative comparison of loop-closure identification in the 
      original and learned feature embedding space}{ The figures show
    the qualitative performance of our proposed localization method
    using the learned embedding (\textit{Ours-fc7}), compared to the
    pre-trained Places365-AlexNet model (\textit{Places365-fc7}). Despite using a naive
    nearest-neighbor strategy, our method is able to minimize false
    positives (crossed-edges shown in red).}
  \seclabel{fig:loop-closure-comparison}
  \vspace{-2mm}
\end{figure}


==> tex/fig-metric-learning-graph-illustration.tex <==
\begin{figure}[!t]
  \centering
  {\renewcommand{\arraystretch}{0.6} %
    {\setlength{\tabcolsep}{4mm}
      \begin{tabular}{M{1.75in}M{1.4in}}
        \includegraphics[scale=0.22]{\SECPROJECTDIR/graphics/siamese-illustration.pdf}
        &\includegraphics[scale=0.22]{\SECPROJECTDIR/graphics/siamese-test-illustration.pdf}\\
        {\scriptsize (a) Training: Siamese Network Architecture}
        & {\scriptsize (b) Testing: Feature embedding} 
          
      \end{tabular}}}
  \mycaption{Training and testing architectures for Siamese
      Networks}{ (a) In a typical siamese network training
      architecture, the CNN weights ($\theta$) are shared between the two
      parallel instantiated graphs, with a common loss (such as the
      contrastive loss) defined between
      them. (b) Once the CNN weights are learned, new features/images
      are mapped into the learned and task-appropriate embedding space $f(\vx_i)$ at test time. }
  \seclabel{fig:metric-learning-graph-illustration}
\end{figure}

